Disentanglement of Correlated Factors via Hausdorff Factorized Support

A grand goal in deep learning research is to learn representations capable of generalizing across distribution shifts. Disentanglement is one promising direction aimed at aligning a model's representation with the underlying factors generating the data (e.g. color or background). Existing disentanglement methods, however, rely on an often unrealistic assumption: that factors are statistically independent. In reality, factors (like object color and shape) are correlated. To address this limitation, we consider the use of a relaxed disentanglement criterion -- the Hausdorff Factorized Support (HFS) criterion -- that encourages only pairwise factorized \emph{support}, rather than a factorial distribution, by minimizing a Hausdorff distance. This allows for arbitrary distributions of the factors over their support, including correlations between them. We show that the use of HFS consistently facilitates disentanglement and recovery of ground-truth factors across a variety of correlation settings and benchmarks, even under severe training correlations and correlation shifts, with in parts over $+60\%$ in relative improvement over existing disentanglement methods. In addition, we find that leveraging HFS for representation learning can even facilitate transfer to downstream tasks such as classification under distribution shifts. We hope our original approach and positive empirical results inspire further progress on the open problem of robust generalization. Code available at https://github.com/facebookresearch/disentangling-correlated-factors.

==> iclr2023/figures/obj_type_adaptation.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{iclr2023/images/adaptation_speed_type_acc.png}
  \end{center}
  \caption{\Karsten{This figure is currently unreferenced.} Adaptation of linear probe to specifically predict object type.}
  \label{fig:obj_type_adaptation}
\end{wrapfigure}

==> iclr2023/figures/toy_example_detailed.tex <==
\begin{figure}
 \centering
 \begin{subfigure}[t]{1\textwidth}
  \begin{center}
    \includegraphics[width=1\textwidth]{iclr2023/images/toy_example_beta_off.png}
  \end{center}
 \caption{VAE with increasing factorization of supports ($\gamma \uparrow$) and prior matching turned off.}  
 \end{subfigure}
 \begin{subfigure}[t]{1\textwidth}
  \begin{center}
    \includegraphics[width=1\textwidth]{iclr2023/images/toy_example_beta_on.png}
  \end{center}
 \caption{$\beta$-VAE with increasing factorization of supports ($\gamma \uparrow$).}
 \end{subfigure}
  \caption{
  \explanation{PREVIOUSLY Fig 2 p 9, NOW MOVED HERE IN APPENDIX }
  \emph{This is a more detailed version and explanation of Fig~\ref{fig:toy_example_simplified}.}
  To illustrate the failures of the assumption of independence and the benefits of our method, we perform a toy experiment. We consider a 2 dimensional dataset, each dimension representing a factor of variation, and where during training the two factors are highly correlated along the diagonal, while the off diagonal samples are under-represented (first column). However at test time (second column) the correlation disappears (specifically, we make every combination equally probable). Training and evaluating a simple $\beta$-VAE (third column), we show in yellow its test reconstructions on top of the ground-truth samples ($\gamma = 0$, i.e. with explicit factorization of the support turned off). We can see the model la\replaced{s}{tc}hes on the diagonal correlation seen at training and poorly generalize outside of the diagonal. From the fourth column onwards, we show the reconstructions using a model trained with increasingly explicit factorization of the support approach, with increasing weight from left to right. We can see that a factorial support assumption rather than factorized distribution allows for a better generalization to test samples.
  \label{fig:toy_example_detailed}
  }
\end{figure}


==> iclr2023/figures/toy_example_simplified.tex <==
\begin{figure}

  \begin{center}
    \includegraphics[width=1\textwidth]{iclr2023/images/toy_example_beta_off.png}
  \end{center}
 \caption{\label{fig:toy_example_simplified}
 \Pascal{Karsten, DON'T WASTE TIME REDOING THIS FIGURE: We NEED TO DISCUSS FIRST}
\added{{\bf Independence v.s. factorized support assumption, 2d toy example.}}
\replaced{We consider a 2 dimensional dataset, ach dimension representing a factor of variation and where during training}{In the training set} the two factors \added{(dimensions)} are highly correlated\replaced{ along the diagonal, while the}{with} off diagonal samples \removed{are} under-represented \removed{(first column)}. \removed{However at test time (second column) the correlation disappears (specifically,} \added{In the test set} we make every combination equally probable. \removed{Training and evaluating a simple $\beta$-VAE (third column),} We show in yellow \removed{its} test reconstructions on top of the ground-truth samples \added{(in blue). We see that a beta-VAE, which assumes factor independence, is fooled by the correlation, and fails to model many off-diagonal modes, reconstructing them instead on the diagonal. Our model, assuming only factorized support, appears far more robust to this. }\removed{($\gamma = 0$, i.e. with explicit factorization of the support turned off). We can see the model latches on the diagonal correlation seen at training and poorly generalize outside of the diagonal. From the fourth column onwards, we show the reconstructions using a model trained with increasingly explicit factorization of the support approach, with increasing weight from left to right. We can see that a factorial support assumption rather than factorized distribution allows for a better generalization to test samples.
A 2D toy distribution with each axis a ground-truth factor. In trainset distribution, the factors are correlated due to underrepresented off-diagonal samples.   (here Beta-VAE) and VAE with increasing factorization of supports ($\gamma \uparrow$) and prior matching turned off.}}  
 \end{figure}
 
%   {\bf Toy example.} Factorization of supports applied to a toy example where certain combination of factors are more likely to co-occur. As can be seen, explicitly encouraging a factorization of support allows for disentanglement and generalization even under correlations in the training data by recovering test modes previously unreachable, both alongside a standard $\beta$-VAE or even as a standalone regularizer.
  
 % To illustrate the failures of the assumption of independence and the benefits of our method, we perform a toy experiment. We consider a 2 dimensional dataset, each dimension representing a factor of variation, and where during training the two factors are highly correlated along the diagonal, while the off diagonal samples are under-represented (first column). However at test time (second column) the correlation disappears (specifically, we make every combination equally probable). Training and evaluating a simple $\beta$-VAE (third column), we show in yellow its test reconstructions on top of the ground-truth samples ($\gamma = 0$, i.e. with explicit factorization of the support turned off). We can see the model lashes on the diagonal correlation seen at training and poorly generalize outside of the diagonal. From the fourth column onwards, we show the reconstructions using a model trained with increasingly explicit factorization of the support approach, with increasing weight from left to right. We can see that a factorial support assumption rather than factorized distribution allows for a better generalization to test samples.


==> iclr2023/tables/btcvae.tex <==
\begin{table}[t]
\begin{subtable}[t]{1\textwidth}
\centering\resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\toprule
Method & No Corr. & Pair: 1 [V1, $\sigma$ = 0.1] & Pairs: 2 [V2, $\sigma$ = 0.1] & Pairs: 3 [V1, $\sigma$ = 0.1] & Conf. [V2, $\sigma$ = 0.2]\\
\hline
$\beta$-VAE & 70.7 \gs{[65.2, 75.4]} & 55.9 \gs{[53.8, 59.0]} & 55.6 \gs{[45.8, 57.2]} & 37.1 \gs{[32.3, 38.9]} & 38.0 \gs{[35.0, 38.6]}\\
$\beta$-TCVAE & 77.1 \gs{[76.6, 78.3]} & 62.0 \gs{[56.6, 64.5]} & 63.8 \gs{[59.1, 65.1]} & 47.3 \gs{[36.7, 50.0]} & 49.9 \gs{[45.8, 55.9]}\\
\hline
$\beta$-TCVAE + \red{\textbf{HFS}}, Optimal $\beta, \gamma$ & \blue{\textbf{85.7 \gs{[82.5, 97.3]}}} & \blue{\textbf{75.2 \gs{[63.1, 76.6]}}} & \blue{\textbf{68.3 \gs{[61.0, 71.8]}}} & \blue{\textbf{51.6 \gs{[47.7, 52.8]}}} & \blue{\textbf{61.5 \gs{[53.8, 64.2]}}}\\
\bottomrule
\end{tabular}
}
\caption{Shapes3D}
\end{subtable}



\begin{subtable}[t]{1\textwidth}
\centering\resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\toprule
Method & No Corr. & Pair: 1 [V2, $\sigma$ = 0.1] & Pairs: 2 [V1, $\sigma$ = 0.1] & Conf. [V2, $\sigma$ = 0.2]\\
\hline
$\beta$-VAE & 32.2 \gs{[25.3, 37.9]} & 9.5 \gs{[7.9, 10.3]} & 7.5 \gs{[6.7, 8.3]} & 11.4 \gs{[9.9, 13.9]}\\
$\beta$-TCVAE & 30.9 \gs{[28.9, 35.2]} & 24.0 \gs{[23.6, 24.4]} & 11.4 \gs{[7.6, 13.6]} & 20.9 \gs{[17.5, 23.6]}\\
\hline
$\beta$-TCVAE + \red{\textbf{HFS}}, Optimal $\beta, \gamma$ & \blue{\textbf{53.1 \gs{[41.8, 53.2]}}} & \blue{\textbf{26.5 \gs{[25.6, 27.2]}}} & \blue{\textbf{27.8 \gs{[16.1, 31.6]}}} & \blue{\textbf{24.8 \gs{[23.8, 26.3]}}}\\
\bottomrule
\end{tabular}
}
\caption{DSprites}
\end{subtable}
\caption{\textit{Benefits of explicit factorization of the support} on top of a $\beta$-VAE extension, $\beta$-TCVAE \citep{chen2018betatcvae}. Again, we find consistent and significant improvements in the disentanglement performance across correlation shifts and benchmarks. Note that we have excluded MPI3D, as we found the standalone factorization of the supports to still perform best (i.e. $\beta$-TCVAE regularization turned off), with values shown in Tab. \ref{tab:main_results}. Note that $\beta$-TCVAE generally outperforms the standard $\beta$-VAE as well as other methods listed in Tab. \ref{tab:main_results}. Still, even here, an explicit factorization of the support offers significant benefits in disentangling across correlations.}
\label{tab:btcvae_plus_fos}
\end{table}

==> iclr2023/tables/mmt_copy.tex <==
\begin{table}[t]
\begin{subtable}[t]{1\textwidth}
\centering
\resizebox{1\textwidth}{!}{
%NoCorr, Pair: 1 [1], Pars: 2 [2], Pairs: 3 [1], Conf. [2]
%NoCorr, Pair: 1[2], Pairs: 2 [1], Conf. [2]
\begin{tabular}{llllll}
\toprule
\textbf{Method} & \textbf{No Corr.} & \textbf{Pairs: 1}, $\sigma$ = 0.1 & \textbf{Pairs: 2}, $\sigma$ = 0.1 & \textbf{Pairs: 3}, $\sigma$ = 0.1 & \textbf{Shared Conf.}, $\sigma$ = 0.2]\\
\hline
$\beta$-VAE & 70.7 \gs{[65.2, 75.4]} & 71.6 \gs{[60.9, 72.5]} & 55.6 \gs{[45.8, 57.2]} & 37.1 \gs{[32.3, 38.9]} & 38.0 \gs{[35.0, 38.6]}\\
\hline
\red{\textbf{HFS}} & 78.3 \gs{[75.1, 83.6]} & 77.8 \gs{[74.4, 78.8]} & 56.0 \gs{[41.0, 57.4]} & 47.5 \gs{[38.0, 49.1]} & 46.2 \gs{[36.3, 47.5]}\\
% $\beta$-VAE + H-FSL, fixed $\beta$ & 81.2 \gs{[76.0, 97.2]} & 64.6 \gs{[57.1, 68.0]} & 80.7 \gs{[78.5, 81.8]} & 81.3 \gs{[75.0, 86.2]} & \blue{\textbf{67.6 \gs{[62.4, 69.3]}}} & 44.9 \gs{[38.9, 45.6]} & 62.8 \gs{[60.2, 64.5]}\\
$\beta$-VAE + \red{\textbf{HFS}} & \blue{\textbf{91.2 \gs{[75.8, 100.0]}}} & \blue{\textbf{80.9 \gs{[76.4, 81.4]}}} & \textbf{67.6 \gs{[62.4, 69.3]}} & \textbf{47.9 \gs{[44.0, 50.8]}} & \blue{\textbf{63.5 \gs{[61.2, 65.5]}}}\\
\hline
$\beta$-TCVAE & 77.1 \gs{[76.6, 78.3]} & 71.1 \gs{[65.5, 72.5]} & 63.8 \gs{[59.1, 65.1]} & 47.3 \gs{[36.7, 50.0]} & 49.9 \gs{[45.8, 55.9]}\\
\hline
$\beta$-TCVAE + \red{\textbf{HFS}} & \textbf{85.7 \gs{[82.5, 97.3]}} & \textbf{75.2 \gs{[63.1, 76.6]}} & \blue{\textbf{68.3 \gs{[61.0, 71.8]}}} & \blue{\textbf{51.6 \gs{[47.7, 52.8]}}} & \textbf{61.5 \gs{[53.8, 64.2]}}\\
\hline
FactorVAE & 66.1 \gs{[51.2, 69.1]} & 70.8 \gs{[70.5, 71.2]} & 57.2 \gs{[55.9, 62.0]} & 46.8 \gs{[40.8, 49.0]} & 31.6 \gs{[27.9, 35.1]}\\
AnnealedVAE & 62.2 \gs{[60.7, 63.2]} & 57.2 \gs{[49.5, 59.3]} & 31.6 \gs{[26.9, 34.1]} & 33.6 \gs{[31.0, 38.0]} & 23.0 \gs{[20.1, 25.9]}\\
\bottomrule
\end{tabular}}
\caption{Shapes3D}
\end{subtable}


%NoCorr, Pair: 1[2], Pairs: 2 [1], Conf. [2]
\begin{subtable}[t]{1\textwidth}
\centering\resizebox{0.87\textwidth}{!}{
\begin{tabular}{l|l|l|l|l}
\toprule
\textbf{Method} & \textbf{No Corr.} & \textbf{Pairs: 1}, $\sigma$ = 0.1 & \textbf{Pairs: 2}, $\sigma$ = 0.1] & \textbf{Shared Conf.}, $\sigma$ = 0.2\\
\hline
$\beta$-VAE & 32.2 \gs{[25.3, 37.9]}  & 9.5 \gs{[7.9, 10.3]} & 7.5 \gs{[6.7, 8.3]} & 11.4 \gs{[9.9, 13.9]}\\
\hline
\red{\textbf{HFS}} & 34.9 \gs{[27.4, 36.0]}  & 13.6 \gs{[7.6, 16.7]} & 11.9 \gs{[9.7, 13.8]} & 15.1 \gs{[11.0, 16.0]}\\
$\beta$-VAE + \red{\textbf{HFS}} & \textbf{49.9 \gs{[30.0, 50.4]}} & 19.7 \gs{[17.0, 21.1]} &  \textbf{17.3 \gs{[6.0, 19.6]}} & 15.8 \gs{[12.3, 16.7]}\\
\hline
$\beta$-TCVAE & 30.9 \gs{[28.9, 35.2]} & \textbf{24.0 \gs{[23.6, 24.4]}} & 11.4 \gs{[7.6, 13.6]} & \textbf{20.9 \gs{[17.5, 23.6]}}\\
\hline
$\beta$-TCVAE + \red{\textbf{HFS}} & \blue{\textbf{53.1 \gs{[41.8, 53.2]}}} & \blue{\textbf{26.5 \gs{[25.6, 27.2]}}} & \blue{\textbf{27.8 \gs{[16.1, 31.6]}}} & \blue{\textbf{24.8 \gs{[23.8, 26.3]}}}\\
\hline
FactorVAE & 25.7 \gs{[20.9, 30.9]} & 15.1 \gs{[11.9, 16.3]} & 13.4 \gs{[12.4, 15.0]} & 14.7 \gs{[13.5, 15.3]}\\
AnnealedVAE & 39.4 \gs{[38.7, 40.0]} & 14.8 \gs{[14.3, 15.9]} & 8.5 \gs{[6.9, 10.3]} & 14.3 \gs{[14.1, 14.5]}\\
\bottomrule
\end{tabular}}
\caption{DSprites}
\end{subtable}



%NoCorr, Pair: 1 [1], Pars: 2 [2], Pairs: 3 [1], Conf. [2]
\begin{subtable}[t]{1\textwidth}
\centering\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\toprule
\textbf{Method} & \textbf{No Corr.} & \textbf{Pairs: 1}, $\sigma$ = 0.1 & \textbf{Pairs: 2}, $\sigma$ = 0.1 & \textbf{Pairs: 3}, $\sigma$ = 0.1 & \textbf{Shared Conf.}, $\sigma$ = 0.2\\
\hline
$\beta$-VAE                             & 25.6 \gs{[24.7, 26.1]} & 20.5 \gs{[17.7, 20.9]} & 23.6 \gs{[22.6, 24.3]} & 11.6 \gs{[11.1, 11.7]} & 11.8 \gs{[10.0, 12.7]}\\
\hline
\red{\textbf{HFS}}                      & \blue{\textbf{32.8 \gs{[30.0, 34.3]}}} & \blue{\textbf{28.4 \gs{[26.5, 29.5]}}} &  \blue{\textbf{28.0 \gs{[27.4, 28.2]}}} & \blue{\textbf{14.3 \gs{[13.1, 14.8]}}} & \blue{\textbf{16.1 \gs{[15.0, 16.6]}}}\\
$\beta$-VAE + \red{\textbf{HFS}}        & \blue{\textbf{32.8 \gs{[30.0, 34.3]}}} & \blue{\textbf{28.4 \gs{[26.5, 29.5]}}} &  \blue{\textbf{28.0 \gs{[27.4, 28.2]}}} & \blue{\textbf{14.3 \gs{[13.1, 14.8]}}} & \blue{\textbf{16.1 \gs{[15.0, 16.6]}}}\\
\hline
$\beta$-TCVAE                           & 26.6 \gs{[26.0, 27.4]} & 20.7 \gs{[20.4, 21.3]} & 23.3 \gs{[21.9, 23.8]} & 11.4 \gs{[10.3, 12.6]} & 14.2 \gs{[13.4, 15.4]}\\
\hline
$\beta$-TCVAE + \red{\textbf{HFS}}      & \blue{\textbf{32.8 \gs{[30.0, 34.3]}}} & \blue{\textbf{28.4 \gs{[26.5, 29.5]}}} &  \blue{\textbf{28.0 \gs{[27.4, 28.2]}}} & \blue{\textbf{14.3 \gs{[13.1, 14.8]}}} & \blue{\textbf{16.1 \gs{[15.0, 16.6]}}}\\
\hline
FactorVAE & 26.0 \gs{[24.8, 27.5]}      & 21.9 \gs{[20.1, 23.9]} & 27.8 \gs{[27.2, 29.2]} & 10.9 \gs{[10.7, 11.9]} & 13.6 \gs{[12.8, 13.9]}\\
AnnealedVAE & 11.8 \gs{[10.8, 12.4]}    & 11.7 \gs{[10.4, 12.9]} & 11.8 \gs{[11.6, 12.1]} & 11.6 \gs{[10.6, 12.2]} & 13.4 \gs{[12.8, 13.9]}\\
\bottomrule
\end{tabular}}
\caption{MPI3D}
\end{subtable}


\caption{\explanation{Merged former Tab. 2, cleaned up table and moved full table to supplementary. Also extended caption text to includemore details.}\textit{Benefits of explicit factorization of the support} for disentanglement as measured using DCI-D across increasing degrees of correlation during training. \blue{\textbf{Boldblue}} denotes best, \textbf{bold} denotes second best performance within a benchmark and correlation settings. \gray{[a, b]} indicates the 25th and 75th percentiles around the median performance, respectively. Every column denotes the number of correlated factors of variations encountered during training, with the total number of correlated factors increasing from left (no correlation, the standard setting) to right (shared confounder - every factor is correlated with one confounding factor). All results are evaluated on the same, uncorrelated test data. 
%%%
The results show that replacing the goal of a factorial latent distribution with that of a \textbf{factorized support offers competitive disentanglement performance} (\red{\textbf{HFS}}). In addition to that, explicitly encouraging a factorized the support \textbf{alongside} a standard disentanglement method ($\beta$-VAE + \red{\textbf{HFS}}) offers even higher improvements, beating out other comparable approaches, in parts by significant margins. In addition to that, we find results to transfer well to other approaches, such as the best performing baseline objective $\beta$-TCVAE. Note that on MPI3D, we found that turning of respective regularizations using only \red{\textbf{HFS}} consistently worked best.}
\label{tab:main_results}
\end{table}



==> iclr2023/tables/supplementary_full_tables.tex <==
\begin{table*}[t]
\caption{shapes3d}\centering\resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\toprule
Method & No Corr. & Pair: 1 [V1, $\sigma$ = 0.1] & Pair: 1 [V2, $\sigma$ = 0.1] & Pair: 1 [V3, $\sigma$ = 0.1] & Pairs: 2 [V1, $\sigma$ = 0.4] & Pairs: 2 [V2, $\sigma$ = 0.4] & Pairs: 2 [V1, $\sigma$ = 0.1] & Pairs: 2 [V2, $\sigma$ = 0.1] & Pairs: 3 [V1, $\sigma$ = 0.1] & Pairs: 3 [V2, $\sigma$ = 0.1] & Conf. [V1, $\sigma$ = 0.2] & Conf. [V2, $\sigma$ = 0.2]\\
\hline
$\beta$-VAE & 70.7 [65.2, 75.4] & 55.9 [53.8, 59.0] & 71.6 [60.9, 72.5] & 66.1 [62.8, 67.0] & 68.5 [56.8, 76.9] & 71.5 [68.1, 75.1] & 58.7 [57.1, 62.9] & 55.6 [45.8, 57.2] & 37.1 [32.3, 38.9] & 40.0 [33.8, 47.5] & 46.8 [42.0, 50.7] & 38.0 [35.0, 38.6]\\
\hline
$\beta$-VAE + H-FSL, $\beta = 0$ & 78.3 [75.1, 83.6] & 56.4 [46.6, 60.2] & 77.8 [74.4, 78.8] & 68.1 [61.2, 69.4] & 73.9 [65.5, 80.0] & 76.7 [69.7, 81.2] & 62.6 [61.2, 64.3] & 56.0 [41.0, 57.4] & 47.5 [38.0, 49.1] & 41.1 [31.7, 42.7] & 51.3 [46.2, 52.5] & 46.2 [36.3, 47.5]\\
$\beta$-VAE + H-FSL, fixed $\beta = 4$ & 81.2 [76.0, 97.2] & 64.6 [57.1, 68.0] & 80.7 [78.5, 81.8] & \blue{\textbf{76.1 [72.2, 79.5]}} & \blue{\textbf{89.1 [78.2, 98.5]}} & 81.3 [75.0, 86.2] & 63.7 [61.0, 65.4] & \blue{\textbf{67.6 [62.4, 69.3]}} & 44.9 [38.9, 45.6] & 52.0 [48.7, 54.5] & 51.7 [50.0, 57.5] & 62.8 [60.2, 64.5]\\
$\beta$-VAE + H-FSL, optimal $\beta, \gamma$ & \blue{\textbf{91.2 [75.8, 100.0]}} & \blue{\textbf{67.3 [59.5, 72.3]}} & \blue{\textbf{80.9 [76.4, 81.4]}} & \blue{\textbf{76.1 [72.2, 79.5]}} & \blue{\textbf{89.1 [78.2, 98.5]}} & \blue{\textbf{83.3 [79.0, 86.5]}} & 65.5 [62.0, 66.6] & \blue{\textbf{67.6 [62.4, 69.3]}} & \blue{\textbf{47.9 [44.0, 50.8]}} & 52.0 [48.7, 54.5] & \blue{\textbf{59.7 [58.6, 62.1]}} & \blue{\textbf{63.5 [61.2, 65.5]}}\\
\hline
$\beta$-TCVAE & 77.1 [76.6, 78.3] & 62.0 [56.6, 64.5] & 71.1 [65.5, 72.5] & 69.8 [67.3, 70.8] & 75.8 [73.0, 79.1] & 75.2 [69.0, 75.9] & \blue{\textbf{65.7 [62.9, 70.0]}} & 63.8 [59.1, 65.1] & 47.3 [36.7, 50.0] & \blue{\textbf{58.1 [56.2, 61.1]}} & 55.9 [52.7, 59.9] & 49.9 [45.8, 55.9]\\
FactorVAE & 66.1 [51.2, 69.1] & 52.2 [44.7, 54.8] & 70.8 [70.5, 71.2] & 65.9 [64.2, 67.8] & 70.2 [64.8, 75.0] & 71.2 [63.0, 77.7] & 62.0 [60.7, 64.5] & 57.2 [55.9, 62.0] & 46.8 [40.8, 49.0] & 40.2 [35.2, 44.6] & 39.2 [34.2, 47.8] & 31.6 [27.9, 35.1]\\
AnnealedVAE & 62.2 [60.7, 63.2] & 39.6 [29.6, 41.6] & 57.2 [49.5, 59.3] & 56.3 [53.0, 57.2] & 60.4 [59.3, 64.9] & 48.5 [39.7, 49.1] & 50.9 [46.0, 52.9] & 31.6 [26.9, 34.1] & 33.6 [31.0, 38.0] & 30.2 [27.1, 30.8] & 26.2 [22.0, 26.8] & 23.0 [20.1, 25.9]\\
\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}[t]
\caption{mpi3d}\centering\resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\toprule
Method & No Corr. & Pair: 1 [V1, $\sigma$ = 0.1] & Pair: 1 [V2, $\sigma$ = 0.1] & Pair: 1 [V3, $\sigma$ = 0.1] & Pairs: 2 [V1, $\sigma$ = 0.4] & Pairs: 2 [V2, $\sigma$ = 0.4] & Pairs: 2 [V1, $\sigma$ = 0.1] & Pairs: 2 [V2, $\sigma$ = 0.1] & Pairs: 3 [V1, $\sigma$ = 0.1] & Pairs: 3 [V2, $\sigma$ = 0.1] & Conf. [V1, $\sigma$ = 0.2] & Conf. [V2, $\sigma$ = 0.2]\\
\hline
$\beta$-VAE & 25.6 [24.7, 26.1] & 15.7 [13.9, 17.0] & 20.5 [17.7, 20.9] & 23.5 [22.5, 24.4] & 23.6 [21.3, 24.7] & 24.8 [24.5, 25.9] & 21.2 [19.5, 21.7] & 23.6 [22.6, 24.3] & 11.6 [11.1, 11.7] & 11.1 [10.9, 11.3] & 15.1 [14.5, 15.8] & 11.8 [10.0, 12.7]\\
\hline
$\beta$-VAE + H-FSL, $\beta = 0$ & \blue{\textbf{32.8 [30.0, 34.3]}} & 20.7 [19.5, 21.2] & \blue{\textbf{28.4 [26.5, 29.5]}} & \blue{\textbf{26.9 [24.7, 28.0]}} & \blue{\textbf{30.1 [29.7, 31.0]}} & \blue{\textbf{30.2 [29.5, 30.5]}} & \blue{\textbf{25.6 [24.0, 26.2]}} & \blue{\textbf{28.0 [27.4, 28.2]}} & \blue{\textbf{14.3 [13.1, 14.8]}} & \blue{\textbf{19.0 [17.8, 19.3]}} & \blue{\textbf{18.9 [14.4, 19.2]}} & \blue{\textbf{16.1 [15.0, 16.6]}}\\
$\beta$-VAE + H-FSL, optimal $\beta, \gamma$ & \blue{\textbf{32.8 [30.0, 34.3]}} & 20.7 [19.5, 21.2] & \blue{\textbf{28.4 [26.5, 29.5]}} & \blue{\textbf{26.9 [24.7, 28.0]}} & \blue{\textbf{30.1 [29.7, 31.0]}} & \blue{\textbf{30.2 [29.5, 30.5]}} & \blue{\textbf{25.6 [24.0, 26.2]}} & \blue{\textbf{28.0 [27.4, 28.2]}} & \blue{\textbf{14.3 [13.1, 14.8]}} & \blue{\textbf{19.0 [17.8, 19.3]}} & \blue{\textbf{18.9 [14.4, 19.2]}} & \blue{\textbf{16.1 [15.0, 16.6]}}\\
\hline
$\beta$-TCVAE & 26.6 [26.0, 27.4] & \blue{\textbf{21.6 [20.4, 23.8]}} & 20.7 [20.4, 21.3] & 23.7 [23.5, 24.2] & 25.6 [25.1, 25.9] & 25.6 [25.4, 26.2] & 21.6 [19.9, 23.2] & 23.3 [21.9, 23.8] & 11.4 [10.3, 12.6] & 16.5 [15.4, 18.2] & 16.7 [16.0, 17.1] & 14.2 [13.4, 15.4]\\
FactorVAE & 26.0 [24.8, 27.5] & 20.1 [15.5, 22.7] & 21.9 [20.1, 23.9] & 24.6 [23.8, 26.2] & 25.0 [24.0, 25.9] & 27.8 [27.2, 29.2] & 21.9 [18.6, 24.0] & 21.6 [17.6, 24.4] & 10.9 [10.7, 11.9] & 15.4 [14.8, 16.4] & 15.5 [15.0, 16.5] & 13.6 [12.8, 13.9]\\
AnnealedVAE & 11.8 [10.8, 12.4] & 10.8 [9.6, 11.9] & 11.7 [10.4, 12.9] & 10.6 [10.3, 11.9] & 12.9 [11.0, 14.8] & 11.8 [11.6, 12.1] & 10.8 [9.8, 11.6] & 12.5 [10.1, 13.5] & 11.6 [10.6, 12.2] & 10.1 [9.8, 11.0] & 13.3 [11.4, 13.8] & 13.4 [12.8, 13.9]\\
\bottomrule
\end{tabular}}
\end{table*}


\begin{table*}[t]
\caption{dsprites}\centering\resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\toprule
Method & No Corr. & Pair: 1 [V1, $\sigma$ = 0.1] & Pair: 1 [V2, $\sigma$ = 0.1] & Pair: 1 [V3, $\sigma$ = 0.1] & Pairs: 2 [V1, $\sigma$ = 0.4] & Pairs: 2 [V1, $\sigma$ = 0.1] & Conf. [V1, $\sigma$ = 0.2] & Conf. [V2, $\sigma$ = 0.2]\\
\hline
$\beta$-VAE & 32.2 \gs{[25.3, 37.9]} & 17.9 \gs{[10.4, 23.0]} & 9.5 \gs{[7.9, 10.3]} & 13.5 \gs{[9.8, 16.1]} & 20.5 \gs{[18.7, 27.6]} & 7.5 \gs{[6.7, 8.3]} & 14.0 \gs{[10.4, 18.5]} & 11.4 \gs{[9.9, 13.9]}\\
\hline
$\beta$-VAE + H-FSL, $\beta = 0$ & 34.9 \gs{[27.4, 36.0]} & 22.7 \gs{[14.4, 25.6]} & 13.6 \gs{[7.6, 16.7]} & 23.3 \gs{[13.8, 28.4]} & 24.1 \gs{[13.3, 30.3]} & 11.9 \gs{[9.7, 13.8]} & 15.8 \gs{[5.4, 18.9]} & 15.1 \gs{[11.0, 16.0]}\\
$\beta$-VAE + H-FSL, fixed $\beta = 2$ & 47.2 \gs{[27.4, 47.4]} & 30.6 \gs{[24.4, 31.6]} & 16.2 \gs{[15.4, 18.4]} & 25.1 \gs{[19.3, 30.8]} & 29.9 \gs{[24.2, 33.4]} & 16.8 \gs{[9.8, 17.5]} & 22.1 \gs{[17.7, 24.4]} & 13.4 \gs{[10.1, 15.6]}\\
$\beta$-VAE + H-FSL, optimal $\beta, \gamma$ & \blue{\textbf{49.9 \gs{[30.0, 50.4]}}} & 32.9 \gs{[21.3, 39.0]} & 19.7 \gs{[17.0, 21.1]} & \blue{\textbf{37.5 \gs{[25.9, 39.1]}}} & \blue{\textbf{38.2 \gs{[21.9, 41.7]}}} & \blue{\textbf{17.3 \gs{[6.0, 19.6]}}} & 22.1 \gs{[17.7, 24.4]} & 15.8 \gs{[12.3, 16.7]}\\
\hline
$\beta$-TCVAE & 30.9 \gs{[28.9, 35.2]} & 35.1 \gs{[32.3, 38.4]} & \blue{\textbf{24.0 \gs{[23.6, 24.4]}}} & 25.0 \gs{[19.0, 30.9]} & 30.2 \gs{[27.9, 42.2]} & 11.4 \gs{[7.6, 13.6]} & \blue{\textbf{29.4 \gs{[28.7, 30.9]}}} & \blue{\textbf{20.9 \gs{[17.5, 23.6]}}}\\
FactorVAE & 25.7 \gs{[20.9, 30.9]} & 22.6 \gs{[20.8, 25.4]} & 15.1 \gs{[11.9, 16.3]} & 21.2 \gs{[19.2, 24.6]} & 21.2 \gs{[13.5, 22.9]} & 13.4 \gs{[12.4, 15.0]} & 18.3 \gs{[17.5, 19.2]} & 14.7 \gs{[13.5, 15.3]}\\
AnnealedVAE & 39.4 \gs{[38.7, 40.0]} & \blue{\textbf{40.8 \gs{[39.4, 41.3]}}} & 14.8 \gs{[14.3, 15.9]} & 29.0 \gs{[26.6, 29.9]} & 30.3 \gs{[28.3, 31.4]} & 8.5 \gs{[6.9, 10.3]} & 19.1 \gs{[18.2, 19.2]} & 14.3 \gs{[14.1, 14.5]}\\
\bottomrule
\end{tabular}}
\end{table*}
